A Study of an Atomic Mobility Game With Uncertainty Under Prospect Theory

In this paper, we present a study of a mobility game with uncertainty in the decision-making of travelers and incorporate prospect theory to model travel behavior. We formulate a mobility game that models how travelers distribute their traffic flows in a transportation network with splittable traffic, utilizing the Bureau of Public Roads function to establish the relationship between traffic flow and travel time cost. Given the inherent non-linearities and complexity introduced by the uncertainties, we propose a smooth approximation function to estimate the prospect-theoretic cost functions. As part of our analysis, we characterize the best-fit parameters and derive an upper bound for the error. We then show the existence of an equilibrium and its its best-possible approximation.

==> notes <==
\begin{lemma}
    A traffic flow $x ^ *$ is a NE if and only if, for all $x \in \mathcal{X}$, for all $i \in \mathcal{I}$, we have $\left \langle \nabla_i c_i(x_i ^ *,x_{- i} ^ *), x_i - x_i ^ * \right \rangle \geq 0$, where by the chain rule with respect to the $x_i ^ {r_i}$ we can take the partial derivatives on the cost function to get
        \begin{equation}
            \left \langle \sum_{r_i \in \mathcal{R}} \sum_{e \in r_i} \sigma'(f_e^*), x_i - x_i^* \right \rangle \geq 0.
        \end{equation}
\end{lemma}

\begin{proof}
    We apply the chain rule with respect to the $x_i^{r_i}$ and substituting the given cost function $c_i(x)$ and flow $f_e(x)$. The traffic flow $x^*$ is a NE if and only if, for all $x \in \mathcal{X}$ and for all $i \in \mathcal{I}$, we have $\left \langle \nabla_i c_i(x_i^*, x_{-i}^*), x_i - x_i^* \right \rangle \geq 0$, where $c_i(x) = \sum_{r_i \in \mathcal{R}} \sum_{e \in r_i} \sigma(f_e)$ and $f_e(x) = \sum_i \sum_{r_i \ni e} x_i^{r_i}$. Now, we compute the gradient of the cost function with respect to $x_i$:
        \begin{equation}
            \nabla_i c_i(x_i^*, x_{-i}^*) = \sum_{r_i \in \mathcal{R}} \sum_{e \in r_i} \frac{\partial \sigma(f_e)}{\partial x_i^{r_i}}.
        \end{equation}
    To compute the partial derivative $\frac{\partial \sigma(f_e)}{\partial x_i^{r_i}}$, we use the chain rule: $\frac{\partial \sigma(f_e)}{\partial x_i^{r_i}} = \sigma'(f_e) \cdot \frac{\partial f_e}{\partial x_i^{r_i}}$,    where $\sigma'(f_e)$ is the derivative of the function $\sigma$ with respect to $f_e$. Since $f_e(x) = \sum_i \sum_{r_i \ni e} x_i^{r_i}$, we have $\frac{\partial f_e}{\partial x_i^{r_i}} = 1$. Now, we can substitute this back into the gradient expression $\nabla_i c_i(x_i ^ *, x_{-i } ^ *) = \sum_{r_i \in \mathcal{R}} \sum_{e \in r_i} \sigma ' (f_e ^ *)$. Finally, we can rewrite the NE condition using the gradient
        \begin{equation}
            \left \langle \sum_{r_i \in \mathcal{R}} \sum_{e \in r_i} \sigma'(f_e ^ *), x_i - x_i ^ * \right \rangle \geq 0.
        \end{equation}
    This is the necessary and sufficient first-order condition for $x_i ^ *$ of any player $i$ to be a minimum of cost function $c_i(\cdot)$.
\end{proof}
